Privacy Perceptions and Behaviors of Google Personal Account Holders in Saudi Arabia

While privacy perceptions and behaviors have been investigated in Western societies, little is known about these issues in non-Western societies. To bridge this gap, we interviewed 30 Google personal account holders in Saudi Arabia about their privacy perceptions and behaviors regarding the activity data that Google saves about them. Our study focuses on Google's Activity Controls, which enable users to control whether, and how, Google saves their Web \& App Activity, Location History, and YouTube History. Our results show that although most participants have some level of awareness about Google's data practices and the Activity Controls, many have only vague awareness, and the majority have not used the available controls. When participants viewed their saved activity data, many were surprised by what had been saved. While many participants find Google's use of their data to improve the services provided to them acceptable, the majority find the use of their data for ad purposes unacceptable. We observe that our Saudi participants exhibit similar trends and patterns in privacy awareness, attitudes, preferences, concerns, and behaviors to what has been found in studies in the US. Our results emphasize the need for: 1) improved techniques to inform users about privacy settings during account sign-up, to remind users about their settings, and to raise awareness about privacy settings; 2) improved privacy setting interfaces to reduce the costs that deter many users from changing the settings; and 3) further research to explore privacy concerns in non-Western cultures.

==> sec/OLD_related.tex <==
\subsection{Privacy Settings Issues} \label{sec:priv_settings_issues}
% lack of awareness
While many web and mobile application providers offer privacy settings to users, users often tend to accept default privacy settings without change. Gross and Acquisti analyzed social media profiles (Facebook) of over 4000 university students~\cite{gross05}. They found that only 1.2\% restricted their profile searchability, and only 0.06\% restricted their profile information visibility. More recently, Malkin et al. surveyed 116 Google and Amazon smart speaker users regarding their attitudes and concerns about voice recordings in their smart speaker devices~\cite{malkin19}. They found that only a minority made use of privacy settings~\cite{malkin19}. For example, 5\% used the device's physical button to mute the microphone~\cite{malkin19}. Of the 44\% who knew about the audio recording review feature, 66.7\% used it only on \quotes{individual occasions,} 17.6\% never used it, and 67.9\% never used the deletion feature~\cite{malkin19}. Lau et al. investigated privacy perceptions, practices, and concerns of smart speaker users~\cite{lau18}. They found that most users did not use the privacy settings of their smart speakers~\cite{lau18}. For example, only two users used the mute button to stop the speaker from listening, and one user deleted audio logs~\cite{lau18}.  \par 
%======================================================================
% privacy settings problems
Researchers identified various awareness and usability issues on privacy settings, such as misconceptions, lack of knowledge, attention, and comprehension. For example, Malkin et al. found that only 48.3\% of participants knew that their audio recordings were saved permanently in their smart speaker devices, while 41.4\% incorrectly believed their recordings were saved temporarily~\cite{malkin19}. Ramokapane et al. interviewed 27 Android and iOS smartphone users to study users' privacy attitudes and concerns regarding smartphone manufacturer provided default settings~\cite{ramokapane19}. They found that most users were not aware of the privacy implications associated with the smartphone manufacturers' default settings~\cite{ramokapane19}. Liu et al.~\cite{liu11} quantified the mismatches between users' actual versus intended privacy settings on 200 Facebook users~\cite{liu11}. They found that privacy settings matched users' intentions only 37\% of the time~\cite{liu11}. Felt et al. investigated users' attention and comprehension of Andriod's permission settings when installing mobile applications~\cite{felt12}. From a survey on 308 participants, and a lab study on 25 Android users, they found that only 17\% of participants paid attention to privacy permission settings during app installation, and only 3\% of the survey participants correctly comprehended the permissions~\cite{felt12}. \par 
%======================================================================
% contributing factors to the problems
Users' lack of awareness and use of privacy settings is in part due to difficulties in finding and configuring them. For example, Ramokapane et al. found that users attributed their failures to configure the mobile phone manufacturer's defaults to \quotes{hidden settings}~\cite{ramokapane19}. Habib et al. surveyed 173 participants and interviewed 25 participants regarding Facebook ad settings~\cite{habib22}. They found that many users found Facebook \quotes{Ad Preferences} difficult to find~\cite{habib22}. Another study by Habib et al. examined websites' opt-out and data deletion choices on 24 participants~\cite{habib20}. They found that participants faced difficulties in finding and using them~\cite{habib20}. Chen et al. examined 100,000 apps' privacy settings using a classifier and found 36.29\% of the privacy settings were classified as \quotes{hidden}~\cite{chen19}. Lau et al. found that multiple users expressed that current privacy settings do not meet their needs~\cite{lau18}. There are a variety of other reasons. For example, lack of knowledge is mentioned among the reasons for users' failures to configure the mobile phone manufacturer's defaults~\cite{ramokapane19}. Another reason is overtrusting the application provider~\cite{zheng18}. On the other hand, losing trust in the application provider can lead users to believe that using privacy settings is useless. For example, Lau et al. reported multiple users expressed doubts that pressing the mute button on their smart speaker would stop the device from listening~\cite{lau18}. Finally, Willis~\cite{willis14} provided a theoretical perspective on the mechanisms that makes default settings \quotes{sticky,} which are: \quotes{transaction barriers,} \quotes{judgment and decision biases,} and \quotes{preference-forming effects of defaults,} which inspired initial a priori themes for our qualitative analysis of the reasons to stick to defaults.

Previous work looked at privacy settings in different contexts: social media, smart home devices, and mobile devices. Despite Google's web applications' popularity and the rich amount of data users share with them, we are not aware of a prior work that investigated Google's personal account \textit{Activity controls} that we investigate. Moreover, most of the existing studies were conducted on western societies, where~\cite{gross05,malkin19,zheng18,lau18,liu11,felt12,habib22,habib20} were in the US,~\cite{ramokapane19} was in the UK, while,~\cite{chen19} was between the US and China. Very limited work studied privacy issues among Arab users in general, and Saudi Arabian users in particular. Moreover, our work provides systematic comprehensive qualitative analysis, which provides new insights at a finer-grained level.
%======================================================================

==> sec/appendices/more_demo.tex <==
\section{Detailed Demographics} \label{app:demo}
~\autoref{tab:demo} provides detailed demographics of the participants.
%============== DEMOGRAPHICS =====================
\begin{table}[!h]
	\centering
	\caption{Participants' general demographics.}
	\label{tab:demo}
    \resizebox{0.35\textwidth}{!}{%
	\begin{tabular}{ll@{\hspace{5pt}}r}
		\toprule
		\multicolumn{3}{c}{\textit{N = 30}} \\
		\hline
		Nationality		& 	\#	&	\%		\\ 
		\hline
		\quad Saudi 	& 25 & (83\%) \\
		\quad Other    	& 5  & (17\%)  \\
		\hline
		%------------------------------------------------------------------------
		Gender			 & 	\#	&	\%	\\
		\hline
		\quad Female 	& 19 & (63\%) \\
		\quad Male    	& 11 & (37\%)  \\
		\hline
		%------------------------------------------------------------------------ 
		Residence region of Saudi Arabia			 & 	\#	&	\%	\\
		\hline
		\quad Western 	 						 & 28 & (93\%) \\
		\quad Eastern	 						 & 0 & (0\%) \\
		\quad Central    						 & 2 & (7\%) \\
		\quad Northern	 						 & 0 & (0\%) \\
		\quad Southern	 						 & 0 & (0\%) \\
		\quad Other (*required: please specify)	 & 0 & (0\%) \\
		\hline 
		%------------------------------------------------------------------------
		Age				&  \#	& \% \\
		\hline
		\quad 18 to 24		& 10 & (33\%) \\
		\quad 25 to 34		& 10 & (33\%) \\
		\quad 35 to 44		& 5 & (17\%) \\
		\quad 45 to 54 		& 5 & (17\%) \\
		\quad 55 to 64 		& 0 & (0\%) \\
		\quad 65 or above	& 0 & (0\%) \\
		\hline 
		%------------------------------------------------------------------------
		Highest degree completed &  \#	& \% \\
		\hline
		\quad Doctorate								&  2   &   (7\%)      \\
		\quad Master's								&  9   &   (30\%)      \\
		\quad Bachelor								&  11  &   (37\%)      \\
		\quad High school							&  8   &   (27\%)      \\
		\quad Intermediate school					&  0   &   (0\%)      \\
		\quad Elementary school						&  0   &   (0\%)      \\
		\quad Other (*required: please specify)		&  0   &   (0\%)      \\
		\hline
		%------------------------------------------------------------------------
		Have CS/IS/IT/CE background?				&  \#	& \% \\
		\hline
		\quad Yes							& 8 & (27\%)\\
		\quad No							& 22 & (73\%) \\
		\hline
		%------------------------------------------------------------------------
		Employment status							&  \#	& \% \\
		\hline
		\quad Student								& 11  & (37\%) \\
		\quad Full-time employee					& 11  & (37\%) \\
		\quad Part-time employee					& 0  & (0\%) \\
		\quad Self-employed or business owner		& 2  & (7\%) \\
		\quad Full-time house wife/husband			& 1  & (3\%) \\
		\quad Unemployed \& looking for a job		& 5  & (17\%) \\
		\quad Unemployed \& not looking for a job   & 0  & (0\%) \\
		\quad Unable to work						& 0  & (0\%) \\
		\quad Retired								& 0  & (0\%) \\
		\quad Other (*required: please specify)		& 0  & (0\%) \\
        \hline
%------------------------------------------------------------------------
		Google account age		& 	\#	&	\%		\\ 
		\hline
		\quad At least since a month  				& 0 & (0\%) \\
		\quad At least since 3 months					& 1 & (3\%) \\
		\quad At least since 6 months					& 2 & (7\%)  \\
		\quad At least since a year					& 2 & (7\%) \\
		\quad At least since 2 years					& 4 & (13\%) \\
		\quad At least since 3 years					& 4 & (13\%) \\
		\quad At least since 5 years					& 4 & (13\%) \\
		\quad At least since more than 5 years 		& 13 & (43\%) \\
		\quad Other (*required: please specify)		& 0  & (0\%) \\
  		\hline
  %------------------------------------------------------------------------
		Browser type		& 	\#	&	\%		\\ 
		\hline
		\quad Google Chrome 		& 22 & (73\%) \\ 
		\quad Firefox				& 2	 & (7\%) \\
		\quad Brave				& 0	 & (0\%) \\
		\quad MS Edge				& 1  &  (3\%) \\
		\quad Safari				& 5  & (17\%) \\
		\quad Opera 				& 0  & (0\%) \\
		\quad Other (*required: please specify)	& 0  & (0\%) \\
		\bottomrule
	\end{tabular}
 } % end resizebox
 \vspace{-10mm}	
\end{table}

\iffalse
%===========BEGIN ACADEMIC BACKGROUND TABLE=============
\begin{table}[!h]
	\centering
	\caption{Employee/Self-Employed participants' academic background based on the latest completed degree.}
	\label{tab:employee_academic_back}
	\begin{tabular}{ll}
		\toprule
		\multicolumn{2}{c}{\textit{N = 13}} \\
		\hline
		Academic background & \#  \\
		\midrule
		Industrial Engineering & 3 \\
		Accounting & 2 \\
		Business Administration & 2 \\
		Administrative Science & 1 \\
		Information Systems & 1 \\
		Computer Science and Artificial Intelligence & 1 \\
		Dentistry & 1 \\
		Pharmacology & 1 \\
		Chemistry & 1 \\
		\bottomrule
	\end{tabular}
\end{table}
%===========END ACADEMIC BACKGROUND TABLE=============

%===========BEGIN WORK SECTORS TABLE=============
\begin{table}[!ht]
	\centering
	\caption{Employee/Self-Employed participants' work sectors.}
	\label{tab:employee_sectors}
	\begin{tabular}{ll}
		\toprule
		\multicolumn{2}{c}{\textit{N = 13}} \\
		\hline
		Work sector & \#  \\
		\midrule
		University Education & 6 \\
		Health & 1 \\
		Media & 1 \\
		Real Estate & 1 \\
		Justice & 1 \\
		Consultancy & 1 \\
		Sales and Retail & 1 \\
		Food Industry & 1 \\
		\bottomrule
	\end{tabular}
\end{table}
%===========END WORK SECTORS TABLE=============

%===========BEGIN STUDENT MAJORS TABLE=============
\begin{table}[!ht]
	\centering
	\caption{Student participants' current academic majors.}
	\label{tab:student_majors}
	\begin{tabular}{ll}
		\toprule
		\multicolumn{2}{c}{\textit{N = 11}} \\
		\hline
		Major & \# \\
		\midrule
		Preparatory Year & 3 \\
		Software Engineering & 1 \\
		Electrical Engineering & 1 \\
		Information Technology & 1 \\
		Computer Science & 1 \\
		Marketing & 1 \\
		Public Administration & 1 \\
		Educational Administration & 1 \\
		Hospitality and Tourism & 1 \\
		\bottomrule
	\end{tabular}
\end{table}
%===========END STUDENT MAJORS TABLE=============

%===========ENGLISH LANG. LEVEL =============
\begin{table}[!ht]
	\centering
	\caption{Participants' English language skills.}
	\label{tab:en_level}
	\begin{adjustbox}{width=\columnwidth}
	\begin{tabular}{ll@{\hspace{5pt}}r}
		\toprule
		\multicolumn{3}{c}{\textit{N = 30}} \\
		\hline
		English level & \# & \% \\
		\hline
		Advanced: I am fluently skilled in English & 4 & (13\%) \\
		Above intermediate: I rarely need to search for English words & 15  & (50\%) \\
		Intermediate: I sometimes need to search for some English words & 6 & (20\%) \\
		Below intermediate: I often need to search for some English words & 5 & (17\%) \\
		Beginner: I know some common English words & 0 & 0\% \\
		I have no English skills at all& 0 & 0\% \\		
		\bottomrule
	\end{tabular}
	\end{adjustbox}
\end{table}		
%=========== END ENGLISH LANG. LEVEL =====================
\fi  


==> sec/appendices/more_discussion.tex <==
\section{Google Steps to Improve Privacy Settings} \label{app:google}
\autoref{fig:updated_ads_settings} and~\autoref{fig:nudge} illustrate some recent Google updates. During and after our study, Google took some steps that are in line with our findings. First, they updated some terms, which support our theme of \quotes{transparency} through \quotes{better presentation} that would have informed unaware users about the data saving~(\autoref{sec:suggestions}). Namely, they updated the term Data \& Personalization to Data \& privacy, and the term Activity Controls to History Settings. Second, Google appears to have started launching nudges about the Activity Controls (~\autoref{fig:nudge}), which comes under the suggestion of \quotes{awareness} through \quotes{notifications or nudges} that would have informed unaware users about data saving~(\autoref{sec:suggestions}).~\autoref{fig:nudge} was first encountered by the main researcher a while after completing the study on Aug. 2022. However, we could not replicate the nudge even if we turned on the Activity Controls. Third, Google also updated their personalized ad settings with more customization (~\autoref{fig:updated_ads_settings}), which accommodates users' attitudes against using their data for Google partners' ads~(\autoref{fig:data_usage_rank}). Having said that, the paper provides other issues that may need Google's attention, such as shorter data retention periods. Moreover, despite Google updates, our results can guide other application providers.

%=========== BEGIN UPDATED AD SETTINGS FIG =====================
\begin{figure} [!th]
	\centering
	\includegraphics[width=0.8\columnwidth]{img/updated_ads_settings}
	\caption{Google's updated ad settings}
	\label{fig:updated_ads_settings}
\end{figure}
%=========== END AUPDATED AD SETTINGS FIG =====================

%=========== BEGIN NUDGES FIG =====================
\begin{figure} [!th]
	\centering
	\includegraphics[width=0.5\columnwidth]{img/nudge}
	\caption{Google's Web \& App Activity nudge.}
	\label{fig:nudge}
\end{figure}
%=========== END NUDGES FIG =====================

==> sec/appendices/more_prefs.tex <==
\section{Further Preferences and Rankings} \label{app:prefs}
~\autoref{tab:retention_rank} shows the participants' preferences (suitability) regarding Google's default retention period.~\autoref{tab:privacy_rank} and~\autoref{tab:sens_rank} show the participants' ranking for the most private and sensitive activity data type.
%================= BEGIN RETENTION PERIOD ATTITUDES TABLE ====================
\begin{table}[h!]
%    \vspace{-5mm}
	\centering
	\caption{Participants' preferences regarding Google's default data retention periods.}
	\label{tab:retention_rank}
    \resizebox{0.5\columnwidth}{!}{%
		\begin{tabular}{lcl@{\hspace{3pt}}rl@{\hspace{3pt}}r}
			
			\toprule
			\multicolumn{6}{c}{N = 29}\\
			\hline
			\multirow{2}{*}{Activity Type} 		& Default Retention Period & \multicolumn{4}{c}{Suitable} \\
			\cline{3-6}
			
			& 		(months)	& \multicolumn{2}{c}{Yes} & \multicolumn{2}{c}{No}  \\
			\hline					   
			Web \& App Activity	 	& 18 mo.		& 8 & (28\%)  & 21 & (72\%) 	  \\
			YouTube History			& 36 mo.		& 4 & (14\%)  & 25 & (86\%) 	  \\
			Location History		 	& 18 mo.		& 6 & (21\%)  & 23 & (79\%) 	   \\
			\bottomrule
			
		\end{tabular}
    } % end resizebox
%\vspace{-5mm}			
\end{table}
%================= END RETENTION PERIOD ATTITUDES 

%\subsection{Rankings of the Most Sensitive and Private Activity Type.} \label{app:opinions}
%We asked all participants to rank the most sensitive and private data type for them (see Q. 26 and Q. 27 in~\autorefappendix{app:questions}). The notions of sensitive and private in these two questions are subjective to each participant. The majority of participants (18/30) ranked Location History data as the most private data type (\quotes{high} privacy degree) and the most sensitive activity data type to them among the three types of activity data. The results are summarized in~\autoref{tab:privacy_rank} and~\autoref{tab:sens_rank} in~\autoref{app:advanced_settings}. It is worth noting that Google's current default for the Location History is turned off (\quotes{paused}) by default. However, while the Location History is turned off by default, the Web \& App Activity description says: \quotes{Saves your activity on Google sites and apps, including associated info like location~\cite{germain22,kang22}.} This confusion regarding how to turn off location tracking by Google recently received public attention in the US~\cite{germain22,kang22}.
%=========================================================
\begin{table}[!h]
	\centering
	\caption{Participants' ranking for the privacy degree for each type of activity data for them. See Q. 26 in~\autorefappendix{app:questions}.}
	\label{tab:privacy_rank}
	\begin{adjustbox}{width=0.5\columnwidth}
		\begin{tabular}{llrlrlr}
			\toprule
            \multicolumn{7}{c}{\textit{N = 30}} \\
			\hline
			\multirow{2}{*}{Data Type} 		& \multicolumn{6}{c}{ Privacy Rank} \\
			\cline{2-7}
			& \multicolumn{2}{c}{High} & \multicolumn{2}{c}{Med} & \multicolumn{2}{c}{Low}\\
			\hline					   
			Web \& App activity	 	& 9 & (30\%) & 19 & (63\%) & 2 & (7\%) \\
			Location History		 	& 18 & (60\%) & 8 & (27\%) & 4 & (13\%)\\
			YouTube History			& 4 & (13\%) & 17 & (57\%) & 9 & (30\%) \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}	
\vspace{-2mm}			
\end{table}
%===============================================================
\begin{table}[!h]
	\centering
	\caption{Participants' ranking for the sensitivity of each type of activity data for them. See Q. 27 in~\autorefappendix{app:questions}.}
	\label{tab:sens_rank}
	\begin{adjustbox}{width=0.5\columnwidth}
		\begin{tabular}{ll@{\hspace{5pt}}rl@{\hspace{5pt}}rl@{\hspace{5pt}}rl@{\hspace{5pt}}r} 
			\toprule
            \multicolumn{9}{c}{\textit{N = 30}} \\
			\hline
			\multirow{3}{*}{Data Type} 				& \multicolumn{8}{c}{Sensitivity Rank} \\
			\cline{2-9}
			& \multicolumn{2}{l}{\makecell{All\\sensitive}} & \multicolumn{2}{l}{\makecell{Some\\sensitive}} & \multicolumn{2}{l}{\makecell{All\\non-Sensitive}} & \multicolumn{2}{c}{Other}\\
			
			\hline					   
			Web \& App Activity 		& 1  & (3\%)  & 25 & (83\%) & 4   & (13\%) & 0 & (0\%) \\
			Location History		 	& 19 & (63\%) & 4  & (13\%) & 7   & (23\%) & 0 & (0\%) \\
			YouTube History			& 2  & (7\%)  & 8  & (27\%) 	  & 20 	& (67\%)	& 0 & (0\%) \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}	
\vspace{-4mm}		
\end{table}

%=========== BEGIN MORE OPTIONS FIG =====================

\section{Acceptable Use of the Web \& App Activity Data}
\autoref{fig:data_usage_rank} shows the participants' preferences regarding the acceptable use of their Web \& App Activity data by Google.
\begin{figure*}[!h]
	\centering
	\includegraphics[width=\textwidth]{img/data_usage_preferences_chart}
	\caption{Participants' preferences regarding the acceptable use of their Web \& App Activity data by Google.}
	\label{fig:data_usage_rank}
%	\vspace{-4mm}	
\end{figure*}
%=========== END MORE OPTIONS FIG =====================


==> sec/appendices/more_related.tex <==
\section{More Background} \label{app:background}
%=========== BEGIN MORE OPTIONS FIG =====================
\begin{figure}[!th] %{r}{0.4\textwidth}
    %\vspace{-8mm}
	\begin{center}
	\includegraphics[width=0.4\textwidth]{img/options}
    \end{center}
	\caption{Google's \quotes{Privacy and Terms} page which appears during the sign-up process. Only if the \quotes{More options} link is clicked, users can change the permissive default privacy settings.}
	\label{fig:options}
	\vspace{-8mm}
\end{figure}
%=========== END MORE OPTIONS FIG ===================== 

==> sec/appendices/more_settings.tex <==
\section{Further Basic Activity Controls Settings vs. Defaults} \label{app:basic_settings}
\autoref{fig:activity_controls_area} shows Google's basic Activity Controls.~\autoref{tab:basic_settings} shows the participants' reported basic Activity Controls settings compare to Google's defaults. See Q.1 in~\autorefappendix{app:questions}.
%============ BEGIN ACTIVITY CONTROLS FIG ===============
\begin{figure}[h!]
    %\vspace{-5mm}
	\begin{center}
	\includegraphics[width=0.4\columnwidth]{img/activity_controls_area}
    \end{center}
	\caption{Google's Activity Controls section.}
	\label{fig:activity_controls_area}
	%\vspace{-5mm}
\end{figure}
%============ END ACTIVITY CONTROLS FIG ===============

%===========BEGIN AC BASIC CHOICES TABLE ==============
%\begin{table}[!t]
\begin{table}[!h] %{r}{0.4\textwidth}
%\vspace{-30mm}
	\centering
	\caption{Participants' basic Activity Controls settings compare to Google's default settings (Q.1 in~\autorefappendix{app:questions}).}
	%The default were captured from a newly created account before the experiment on Jul. 20, 2021.
	\label{tab:basic_settings}
	\resizebox{0.5\columnwidth}{!}{%
		\begin{tabular}{lll@{\hspace{5pt}}rl@{\hspace{5pt}}r}
			\toprule
			\multicolumn{6}{c}{\textit{N = 30}} \\
			\hline
			\multirow{2}{*}{Data Type} & \multirow{2}{*}{Default Settings} & \multicolumn{4}{c}{Participants' Settings} \\
			\cline{3-6}
			&  & \multicolumn{2}{c}{On} & \multicolumn{2}{c}{Paused} \\
			\hline					   
			Web \& App Activity	& On 		& 28/30 & (93\%) & 2/30 & (7\%) \\
			Location History		& Paused 	& 10/30 & (33\%) & 20/30 & (67\%) \\
			YouTube History		& On 		& 28/30 & (93\%) & 2/30 & (7\%) \\
			\bottomrule
		\end{tabular}
	} % resizebox
%\vspace{-5mm}
\end{table}
%\end{table}
%===========END AC BASIC CHOICES TABLE ============== 

\section{Further Advanced Activity Controls Settings vs. Defaults} \label{app:advanced_settings}
~\autoref{tab:advanced_settings} shows the participants' reported advanced Activity Controls options compare to Google's defaults. See Q.8 in~\autorefappendix{app:questions}.~\autoref{tab:autodelete_settings} shows the participants' reported auto-delete settings compare to Google's defaults. See Q.9 and Q.10 in~\autorefappendix{app:questions}.
%===============BEGIN ADVANCED AC SETTINGS TABLE=======================
\begin{table*}[!h]
	\centering
	\caption{Participants' Web \& App Activity and YouTube History Activity Controls advanced options (see Q. 8 in~\autorefappendix{app:questions}). \textit{N} represents the participants who reported one or more activity data types in their Activity Controls settings are \quotes{on.} We omitted the Location History settings as the Location History did not have any advanced options (check-boxes), and we did not proceed to the Location History advanced settings with any participant.}
	\label{tab:advanced_settings}
    \resizebox{0.8\textwidth}{!}{%
	\begin{tabularx}{\textwidth}{lX|c|cc|cc}
		\toprule
		\multicolumn{7}{c}{\textit{N = 29}} \\
		\hline
		\multirow{2}{*}{Data Type} & \multirow{2}{*}{Options} & \multirow{2}{*}{Default Settings} & \multicolumn{4}{c}{Participants' Settings} \\
		\cline{4-7}
		& 						&  						 & \multicolumn{2}{c}{checked} & \multicolumn{2}{c}{unchecked}   \\ 
		\cline{4-7}
		& 						&  						 & \# & \% & \# & \%  \\
		\midrule
		\multirow{2}{*}{Web \& App Activity} 
		& \tabitem Include Chrome history and activity from sites, apps, and devices that use Google services  & checked	 & 24
		/28 & (86\%)  & 4/28 & (14\%) \\
		\cline{2-7}
		& \tabitem Include audio recordings 																   	& unchecked  	 & 0/28  & (0\%) & 28/28 & (100\%)  \\
		
		\midrule
		\multirow{2}{*}{YouTube History}   	 
		& \tabitem Include the YouTube videos you watch 													    & checked 	& 1/1 & (100\%) & 0/1 & (0\%) \\
		\cline{2-7}
		& \tabitem Include your searches on YouTube 															& checked	& 1/1 & (100\%) & 0/1 & (0\%) \\
		\bottomrule
	\end{tabularx}
    } % end tabularx
\end{table*}
%===============END ADVANCED AC SETTINGS TABLE=======================

%===============BEGIN AUTODELETE SETTINGS TABLE=======================
\begin{table*}[!h]
	\centering
	\caption{Participants' Auto-delete and retention period settings in Google's Activity Controls. See Q.9 and Q.10 in~\autorefappendix{app:questions}. Note that the retention period is applicable only if the Auto-delete setting is \quotes{on.} \textit{N} represents the participants who reported one or more activity data types in their Activity Controls settings are \quotes{on.} We omitted the Location History settings as we did not need to proceed to it with any of our participants.}
	\label{tab:autodelete_settings}
	\resizebox{0.8\textwidth}{!}{%
		\begin{tabularx}{\textwidth}{lll|lr|lr|lr|lr|lr} 
			\toprule
			\multicolumn{13}{c}{\textit{N = 30}} \\
			\hline
			\multirow{3}{*}{Data Type}   & \multicolumn{2}{c}{Default Settings}  & \multicolumn{9}{c}{Participants' Settings}\\
			\cline{2-3}\cline{4-13}
			& \multirow{2}{*}{Status} &	\multirow{2}{*}{Delete Every}  & \multicolumn{4}{c}{Status}  & \multicolumn{6}{c}{Delete Every} \\
			
			\cline{4-13}			
			& 			&              & \multicolumn{2}{c}{On}  & \multicolumn{2}{c}{Off}  & \multicolumn{2}{c}{3 mo.}& \multicolumn{2}{c}{18 mo.}& \multicolumn{2}{c}{36 mo.} \\ 
			
			\midrule
			& 			&              & \# & \% & \# & \% & \# & \% & \# & \% &  \# & \% \\
			\cline{4-13}
			
			Web \& App Activity & \quotes{On} 			&  18 mo.      & 6/28 & (21\%) & 22/28 & (79\%)	 	& 4/6 & (67\%)  & 2/6 & (33\%) & 0/6 & (0\%)  \\
			
			
			\midrule
			
			YouTube History	 & \quotes{On} 			&  36 mo.     & 1/1  & (100\%) &  0/1  & (0\%) 	& 1/1  & (100\%) & 0/1  & (0\%) & 0/1 & (0\%) \\
\hline
            & Total& & 7/29 & (24\%) & 22/29 & (76\%) & 5/7 & (71\%) & 2/7 & (29\%) & 0/7 & (0\%) \\
			\bottomrule   
		\end{tabularx}
	}% resizebox
%\vspace{-4mm}	
\end{table*}
%===============END AUTODELETE SETTINGS TABLE======================= 

%\subsection{Knowledge and Usage of the Review, Delete, and Auto-delete Features.} \label{app:awarenss_use_data_saving} 
%We asked the 10  participants who answered \quotes{yes,} they know that Google saves data about them,\footnote{An additional participant said \quotes{yes} to this questions, but missed~\autoref{sec:awarenss_use_data_saving}'s questions due to an error.} whether they knew that they can review the data that Google saves about them (see Q. 15 in~\autorefappendix{app:questions}). 5/10 answered \quotes{yes} (4 in the Web \& App Activity, and 1 in the YouTube History groups), while the remaining participants answered \quotes{no.} We asked them how often they review the data (see Q. 16 in~\autorefappendix{app:questions}). 3/5 answered \quotes{at least once every 6 months,} one answered \quotes{less than once a year,} and one answered \quotes{I never reviewed them.} We asked the same 10 participants who said they knew Google saves data about them whether they knew they can manually delete some or all the data that Google saves about them (see Q. 17 in~\autorefappendix{app:questions}), and whether they knew about the Auto-delete feature (see Q. 19 in~\autorefappendix{app:questions}). 7/10 said they knew they could manually delete data,  and only 3/10 said they knew about Auto delete. Of the 7 who said they knew about manual deletion, we asked them how often they manually delete their data (see Q. 18 in~\autorefappendix{app:questions}). We find 4/7 said they \quotes{never deleted them,} and 2/7 \quotes{do not remember.} 

%====================================================================================


==> sec/appendices/questions_closing.tex <==
\subsection{Closing Questions}
\begin{itemize}
\item \textbf{Q.} Do you have any degree or work on the cyber security area? \par
	\textbf{Answers:} \begin{inparaitem}[$\circ$] \item \quotes{Yes,} \item \quotes{No}  \end{inparaitem}
\vspace{4pt}
\item \textbf{Q.} Do you believe you learned something from the interview?\par 
	\textbf{Answers:} Open
\vspace{4pt}
\item \textbf{Q.} Are there any questions you expected us to ask you? \par 
    \textbf{Answers:} Open
\vspace{4pt}
\item \textbf{Q.} Are there any additional information related to the interview topic you would like to say? \par 
    \textbf{Answers:} Open
 \vspace{4pt}   
\item \textbf{Q.} Can you nominate other participants? \par
    \textbf{Answers:} Open
\end{itemize}
%-------------------------------------------------

==> sec/appendices/questions_demo.tex <==
\subsection{Demographic Questions}
\begin{itemize}
    \item \textbf{Q. 1} What is your nationality?  \par
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Saudi,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par 
    \vspace{4pt}

    \item \textbf{Q. 2} What is your gender? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Female,} \item \quotes{Male} \end{inparaitem} \par  
    \vspace{4pt}

    \item \textbf{Q. 3} What is your marital status? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Single,} \item \quotes{Married,} \item \quotes{Divorced,} \item \quotes{Widow,} \item \quotes{I prefer not to answer,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par  
    \vspace{4pt}

    \item \textbf{Q. 4} Do you have kids? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Yes,} \item \quotes{No,} \item \quotes{I prefer not to answer,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par  
    \vspace{4pt}

    \item \textbf{Q. 5} Where do you live?  \par
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Saudi Arabia,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par 
    \vspace{4pt}

    \item \textbf{Q. 6} In which region of Saudi Arabia do you live?  \par
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Western,} \item \quotes{Eastern,} \item \quotes{Central,} \item \quotes{Northern,} \item \quotes{Southern,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par 
    \vspace{4pt}

    \item \textbf{Q. 7} What is the highest academic degree you completed?  \par
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Doctorate,} \item \quotes{Masters,} \item \quotes{Bachelor,} \item \quotes{High school,} \item \quotes{Middle school,} \item \quotes{Elementary school,} \item \quotes{Other (*required: please specify)} \end{inparaitem} \par 
    \vspace{4pt}

    \item \textbf{Q. 8} \textbf{[If Q. 7 answer was \quotes{Doctorate}]} What is your major for the Doctorate degree? \par
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 9} \textbf{[If Q. 7 answer was \quotes{Doctorate} or \quotes{Masters}]} What is your major for the Masters degree? \par
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 10} \textbf{[If Q. 7 answer was \quotes{Doctorate} or \quotes{Masters} or \quotes{Bachelor}]} What is your major for the Bachelor degree? \par
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 11} \textbf{[If Q. 7 answer was \quotes{Doctorate} or \quotes{Masters} or \quotes{Bachelor}]} What is your major for the Bachelor degree? \par
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 12} What is your current employment status? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Student,} \item \quotes{Full-time employee,} \item \quotes{Part-time employee,} \item \quotes{Self-employed or business owner,} \item \quotes{Full-time house wife/husband,} \item \quotes{Unemployed, and looking for a job,} \item \quotes{Unemployed and, and not looking for a job,} \item \quotes{Unable to work,} \item \quotes{Retired,} \item \quotes{Other (*required: please specify)} \end{inparaitem}\par 
    \vspace{4pt}

    \item \textbf{Q. 13} \textbf{[If Q. 12 answer was \quotes{Student}]} If you are a student, what is the degree you are currently studying? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Doctorate,} \item \quotes{Masters,} \item \quotes{Bachelor,} \item \quotes{High school,} \item \quotes{Other (*required: please specify)} \end{inparaitem}\par 
    \vspace{4pt}

    \item \textbf{Q. 14} \textbf{[If Q. 12 answer was \quotes{Student} and Q. 13 answer was \quotes{Doctorate}]} What is the major you are currently studying in the Doctorate degree?
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 15} \textbf{[If Q. 12 answer was \quotes{Student} and Q. 13 answer was \quotes{Masters}]} What is the major you are currently studying in the Masters degree?
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 16} \textbf{[If Q. 12 answer was \quotes{Student} and Q. 13 answer was \quotes{Bachelor}]} What is the major you are currently studying in the Bachelor degree?
    \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 17} Do you have a degree or work on Computer Science, Information Systems, Information Technology, or Computer Engineering? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Yes,} \item \quotes{No} \end{inparaitem} \par 
    \vspace{4pt}

    \item \textbf{Q. 18} \textbf{[If Q. 12 answer was \quotes{Full-time employee} or \quotes{Part-time employee} or \quotes{Self-employed or business owner}]} What is the sector you are currently working on? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Education (pre-university),} \item \quotes{University Education,} \item \quotes{Health,}  \item \quotes{Communication and Information Technology,} \item \quotes{Financial,} \item \quotes{Industrial,} \item \quotes{Agricultural,} \item \quotes{Sales and retail,} \item \quotes{Petrochemical,} \item \quotes{Other (*required: please specify)}  \end{inparaitem} \par 
    \vspace{4pt}
    
    \item \textbf{Q. 19} \textbf{[If Q. 12 answer was \quotes{Retired}]} What is the sector you worked on for your last job? \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Education (pre-university),} \item \quotes{University Education,} \item \quotes{Health,}  \item \quotes{Communication and Information Technology,} \item \quotes{Financial,} \item \quotes{Industrial,} \item \quotes{Agricultural,} \item \quotes{Sales and retail,} \item \quotes{Petrochemical,} \item \quotes{Other (*required: please specify)}  \end{inparaitem} \par 
    \vspace{4pt} \par 

    \item \textbf{Q. 20} \textbf{[If Q. 12 answer was \quotes{Full-time employee} or \quotes{Part-time employee} or \quotes{Self-employed or business owner}]} What is your current job title? (e.g. Teacher, Assistant Professor, Doctor, Nurse, etc.)? \par
   \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 21} \textbf{[If Q. 12 answer was \quotes{Retired}]} What is your job title in your last job? (e.g. Teacher, Assistant Professor, Doctor, Nurse, etc.)? \par
   \textbf{Answers:} Open	\par 
    \vspace{4pt}

    \item \textbf{Q. 22} What is your rate for your English language proficiency level?
    \par 
    \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Advanced (fluent in English),} \item \quotes{Above average (I rarely need to search for words),} \item \quotes{Average (Sometimes I need to search for some words),} \item \quotes{Below average (Mostly, I need to search for some words),} \item \quotes{Beginner (I know some common words),} \item \quotes{I do not know English at all} \end{inparaitem}

    \item \textbf{Q. 23} Approximately, when did you start using this email (that you used in the interview experiment)? \par 
     \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{At least since a month,} \item \quotes{At least since 3 months,} \item \quotes{At least since 6 months,} \item \quotes{At least since a year,} \item \quotes{At least since 2 years,} \item \quotes{At least since 3 years,} \item \quotes{At least since 4 years,} \item \quotes{At least since 5 years,} \item \quotes{At least since more than 5 years,} \item \quotes{Other (*required: please specify)}\end{inparaitem}

    \item \textbf{Q. 24} What is the browser that you mostly use when you browse the Internet? \par 
     \textbf{Answers:} \begin{inparaitem}[$\circ$]\item \quotes{Google Chrome,} \item \quotes{Firefox,} \item \quotes{Brave,} \item \quotes{MS Edge,} \item \quotes{Safari,} \item \quotes{Opera,} \item \quotes{Other (*required: please specify)}\end{inparaitem}
     
\end{itemize}
